Chain of Draft: Thinking Faster by Writing Less

Large Language Models (LLMs) have demonstrated remarkable performance in solving complex reasoning tasks through mechanisms like Chain-of-Thought (CoT) prompting, which emphasizes verbose, step-by-step reasoning. However, humans typically employ a more efficient strategy: drafting concise intermediate thoughts that capture only essential information. In this work, we propose Chain of Draft (CoD), a novel paradigm inspired by human cognitive processes, where LLMs generate minimalistic yet informative intermediate reasoning outputs while solving tasks. By reducing verbosity and focusing on critical insights, CoD matches or surpasses CoT in accuracy while using as little as only 7.6% of the tokens, significantly reducing cost and latency across various reasoning tasks. Our code and data are available at https://github.com/sileix/chain-of-draft.

==> sections/ablation.tex <==
\subsection{Ablation Study}
\subsubsection{Total Budget vs Per-Step Budget}


\subsubsection{How Many Words Do We Need}
In previous experiments, we instruct LLMs to limit the reasoning steps to 5 words at most. In this section, we conduct ablation study on what is the optimal word limit. 

\subsubsection{CoD on Different Model Sizes}
To understand how CoD performs on models with different sizes, we also evaluate GSM8K with Llama 3.1 8B, 70B, and 405B~\cite{llama3.1}.

